PICProp: Physics-Informed Confidence Propagation for Uncertainty Quantification

Standard approaches for uncertainty quantification in deep learning and physics-informed learning have persistent limitations. Indicatively, strong assumptions regarding the data likelihood are required, the performance highly depends on the selection of priors, and the posterior can be sampled only approximately, which leads to poor approximations because of the associated computational cost. This paper introduces and studies confidence interval (CI) estimation for deterministic partial differential equations as a novel problem. That is, to propagate confidence, in the form of CIs, from data locations to the entire domain with probabilistic guarantees. We propose a method, termed Physics-Informed Confidence Propagation (PICProp), based on bi-level optimization to compute a valid CI without making heavy assumptions. We provide a theorem regarding the validity of our method, and computational experiments, where the focus is on physics-informed learning.

==> tex/experiment/allen_cahn.tex <==
\subsection{Two-dimensional, steady-state Allen-Cahn equation}

Finally, we consider a steady-state version of Allen-Cahn equation given as

\begin{equation}
\begin{gathered}
c\cdot((u_x)^2 + (u_y)^2) + u(u^2-1) = f, \quad (\text{P.D.E.}), \quad (x, y) \in [-1, 1] \times [-1, 1], \\
u(x, y) = 0, \quad (\text{B.C.}).
\end{gathered}
\label{eq:allen_cahn}
\end{equation}

where $c=0.01$ represents the mobility.
The exact solution is set to be $u(x, y) = \sin(\pi x) \cdot \sin(\pi y)$ and the corresponding $f(x, y)$ can be obtained. 
The boundary conditions are

\begin{equation}
    \begin{gathered}
        u(x=-1, y\neq\pm1) \sim \mathcal{N}(0, \sigma),\\
        u(x=1, y) = u(x \neq -1, y=-1) = u(x \neq -1, y=1) = 0 \\
    \end{gathered}
    \label{eq:allen_cahn_bc}
\end{equation}

where $\sigma=0.05$. 
For this example, we propagate a fixed and given CI, $u(x=-1, y\neq\pm1) \in [-0.098, 0.098]$. 
A two-layer fully connected neural network of which each hidden layer has 32 units is used for both the PINN and CIML models. 
50 boundary points are sampled for each edge i.e., there are 200 boundary points in total for training but uncertainty only occurs at 50 points. 
1000 boundary conditions within the given CI are sampled for exhaustive search. 
10000 residual points for PINN training and 441 query points for CIML are sampled in a grid-mesh manner. 
For meta-optimization, the method to compute hyper-gradient is \emph{Reverse}, and the meta-optimizer is \emph{SGD} with learning rate $0.01$.
The number of inner steps for each meta-step is set to be 500, which results in ~1 second per meta step. 
100 meta-steps are run for upper/lower CI bound for each query. 
CI predictions of exhaustive search and CIML are plotted in Fig.~\ref{fig:allen_cahn_ci}. Slices of the bounds predicted by CIML-efficient at $x (or y) = -1.0, -0.5, 0.0, 0.5$ are plotted in Fig.~\ref{fig:allen_cahn_ci_x} and Fig.~\ref{fig:allen_cahn_ci_y} respectively.

\begin{figure}[H]
    \centering
    \includegraphics[width=1.0\linewidth]{img/allen-cahn/bo/allen-cahn.pdf}
    \caption{\textbf{Allen-Cahn equation}: The heat maps of upper and lower boundaries predicted by the exhaustive search and CIML-efficient methods.}
    \label{fig:allen_cahn_ci}
\end{figure}


\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{img/allen-cahn/bo/allen-cahn-x.pdf}
    \caption{\textbf{Allen-Cahn equation}: Slices of the bounds predicted by CIML-efficient at $x=-1.0, -0.5, 0.0, 0.5$}
    \label{fig:allen_cahn_ci_x}
\end{figure}


\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{img/allen-cahn/bo/allen-cahn-y.pdf}
    \caption{\textbf{Allen-Cahn equation}: Slices of the bounds predicted by CIML-efficient at $y=-1.0, -0.5, 0.0, 0.5$}
    \label{fig:allen_cahn_ci_y}
\end{figure}

==> tex/revision_todos.tex <==
\section{Revisions required}

% TODO 1,  Reviewer H2bG.
% Regarding revision, we will follow the reviewer's suggestions to (1) enhance the comprehensiveness of the relevant discussions in the introduction and (2) revise other parts of the manuscript where there might be statements that inadvertently suggest "Wide CI = safety," including but not limited to line 285, line 309 and the caption of Figure 5.

% TODO 2, Reviewer Lv8K (and also Reviewer Jho9).
% To Q3: The dimensionality of PDE/ODE problems is typically N+1, where N is the number of spatial dimensions and 1 accounts for the temporal dimension. In this regard, the problems that we considered in this paper involve standard representative equations met in many real-world problems including heat transfer, fluid dynamics, flows through porous media, and even epidemiology [\cite{meng2021multi, zou2022neuraluq}] and N is in many practical cases equal to 1 or 2. The problems that we selected to present in this paper are similar to or the same as the standard problems solved by the computational science community for developing novel solution methods (both deterministic [\cite{psaros2022meta}] and considering uncertainty [\cite{yang2019adversarial}]).

% We thank the reviewer for the comment and we would like to add some clarifications to our previous comment. Please note that the cases that we considered in the paper can already be viewed as real-world applications. For example, the Burgers equation is often used as a simplified version of the Navier-Stokes equation for fluid mechanics applications.

% TODO 3, Reviewer Jho9.
% For future work, see Weakness 3 by reviewer: As of now, the proposed method only propagates uncertainty from boundary points.

% PICProp can be easily generalized to propagate uncertainty from inner data points or collocation data points, once CIs/data to construct CIs at these points are available. We plan to work on it in the future.
% NOTE: Added a sentence "(at the boundary but can easily be extended to  inner or collocation data points)" in brackets in Section 6 Conclusion.

% We are not doing this. I believe that the disadvantages of doing this outweigh the advantages.
% TODO 4, Reviewer JUgH.
% Q3: Please consider discussing the Bayesian PINNs in the main text.
% To Weakness 2 and Q3: We thank the reviewer for the revision suggestion. We will accordingly move some of that discussion into the main text in the revised manuscript.

% TODO 5, Reviewer JUgH.
% Q2: In appendix C, you should mentioned the well-known result of Jensen's inequality as the figures are an illustration of this.
% To Q2: We thank the reviewer for the constructive suggestion. We will mention Jensen's inequality in the revised manuscript.
% NOTE: Added a sentence "The convex (and concave) functions are essentially Jensen's inequality." at the end of the paragraph in Appendix C.

% TODO 6, Reviewer 5z2U.
% Q1: In eqn. (5) it seems that the lower and upper boundary data points should be derived by finding the points that minimized $u_{\hat{\theta}}(x)$ at $x = x_q^k$ rather than for all $x$. Is that correct?
% To Q1: The reviewer is right. We will correct this typo in the revised manuscript.

% TODO 7, Reviewer 5z2U.
% Q2: Four lines above eqn. (4), should z minimize (rather than maximize) the corresponding value to determine L(x)?
% To Q2: We assume the reviewer meant "Four lines above eqn. (5)". The reviewer is right. We will correct this typo in the revised manuscript.

% TODO 8, Reviewer 5z2U.
% Q3: Third to last last line of section 4, SimPICProp is not defined in the main paper. It may be better to state that SIMPICProp is the version of EffPICProp where $\lambda = 0$.
% To Q3: Thanks for the reviewer's suggestion. We use the term "SimPICProp" for the naive regression approach to distinguish it from the meta-learning approach, EffiPICProp (). We will consider the reviewer's suggestion for revision.

% TODO 9, Reviewer 5z2U.
% Q4: The paper use the term confidence interval for Def. 3.1. Based on the work of Ramdas, I believe this is a confidence sequence. The authors should verify if this is indeed the case.
% To Q4: By CI in Def. 3.1, we meant joint confidence interval, which is exactly confidence sequence, to the best of the authors' knowledge. We use the term (joint) confidence interval as it is commonly used in the literature ([27][29][19]). For revision, we will cite the work of Ramdas and point out the equivalence between confidence sequence and joint confidence interval. We will also modify Def. 3.1 to avoid ambiguity.

% TODO 10, Reviewer 5z2U. Weakness 2:
% We thank the reviewer for pointing out this crucial issue. We conducted the following experiment to address the reviewer's concern about the validity of CIs. ...

% Due to the limited time, we will add more results in a later revision.
